EREBA: Black-box Energy Testing of Adaptive Neural Networks

Recently, various Deep Neural Network (DNN) models have been proposed for environments like embedded systems with stringent energy constraints. The fundamental problem of determining the robustness of a DNN with respect to its energy consumption (energy robustness) is relatively unexplored compared to accuracy-based robustness. This work investigates the energy robustness of Adaptive Neural Networks (AdNNs), a type of energy-saving DNNs proposed for many energy-sensitive domains and have recently gained traction. We propose EREBA, the first black-box testing method for determining the energy robustness of an AdNN. EREBA explores and infers the relationship between inputs and the energy consumption of AdNNs to generate energy surging samples. Extensive implementation and evaluation using three state-of-the-art AdNNs demonstrate that test inputs generated by EREBA could degrade the performance of the system substantially. The test inputs generated by EREBA can increase the energy consumption of AdNNs by 2,000% compared to the original inputs. Our results also show that test inputs generated via EREBA are valuable in detecting energy surging inputs.

==> Preliminary.tex <==
\section{Preliminary Findings}
\label{sec:prelim}
We have generated some empirical results which indicates the difficulty to establish relations between input to a DNN model and energy consumption of that model. Although, traditional DNNs requires same number of computations for every input, the energy consumption could still be different for different computations. Because of this intuition, we have measured energy consumption of three traditional DNN models with Caffe framework using Nvidia TX2 server. The three models we have chosen are - AlexNet, GoogLeNet and ResNet. These three models use significantly different number of computations to process images. 

  To investigate a relation between energy consumption and input, we perform two type of experiments.
  First, we classify 10000 collected images from Wikipedia dataset using the above mentioned three models and measure the energy consumption. This experiment is to know if a particular type (\textit{e.g.,} clear or unclear objects, dark or bright background)  of image is consuming more energy than others. 
 Second, we selected 1000 images from 10000 initial wikipedia images and transform those image by increasing or decreasing color, brightness and contrast to different levels. We classify these transformed images to know if adding noise to image pixels can change the energy consumption.

To remove anomalies, we infer each image for five times and remove the energy consumption entries which are more than twenty percent different than other recorded entries. Then, we took the average of the non-discarded entries.  Table \ref{tab:enrg} represents maximum and minimum energy consumption for an image inference of three models. From the results, we can find that the range of energy consumption for all the images for a particular DNN is within 20 percent of the highest value.

 For the second type of experiments, we found that it is difficult to find a pattern if a particular type of transformation consumes more amount of energy than other transformations. For example, increasing brightness for one image can increase the energy consumption for that image. Although, for a different image, increasing brightness would decrease energy consumption. 
 
 From these results, it becomes difficult to indicate that if the energy consumption is only dependent on computations or not. The 20 percent difference in energy consumption could be result of different hardware specifications. Other than that, incapability of finding pattern from second set of experiments makes it difficult to formulate any attack technique. 
 

 

%\begin{center}
\begin{table}[t]
		\scriptsize\center\caption{\label{tab:enrg} Maximum and Minimum energy consumption of Different Models} 
 \begin{tabular}{||c | c |c||} 
 \hline
 Model & Maximum Energy (mJ) & Minimum Energy (mJ) \\ [0.5ex] 
 \hline\hline
 AlexNet & 174 & 192 \\ 
 \hline
 GoogLeNet & 217 & 241  \\
 \hline
 ResNet & 710 & 800  \\
 \hline
 
\end{tabular}
\end{table}

==> background.tex <==



\section{Background}
\label{sec:back}
\begin{comment}

\begin{figure}[t]%
	\centering
	\includegraphics[width=0.47\textwidth]{figures/AdNN Architechture.pdf}
    \caption{Working mechanism of a AdNN}
	\label{fig:example3}
\end{figure}
\end{comment}
In this paper, we focus on evaluating the energy robustness of AdNNs. The main objective of AdNNs is to avoid executing a few layers in a Neural Network. The AdNNs produce intermediate outputs before each layer or block (in the case of ResNet). \cite{MirazILFO}
A shallow computing unit (linear classifier or simple CNN, RNN) is generally added between two layers or blocks to calculate intermediate outputs. Predefined conditions are used to evaluate these intermediate outputs, and if output attains a certain threshold, the condition is fulfilled.
After fulfilling the condition, if AdNN decides that certain layers or blocks are not required for the inference and those layers or blocks are skipped.
That type of AdNN is called  \textit{Conditional-skipping AdNN} \cite{wang2018skipnet,wu2018blockdrop}. Otherwise, if AdNN terminates the operations within a block or network early by deciding that later part of the operations are not required, then we call those AdNNs as \textit{Early-termination AdNNs} \cite{figurnov2017spatially,bolukbasi2017adaptive}.
 

%\Cong{Need a rewrite. You are targeting at different AdNNs now. Also important to convince why only studying these three models are sufficient.}

In section~\ref{sec:eval}, we evaluate our work on three popular open-source AdNNs: SkipNet~\cite{wang2018skipnet}, BlockDrop~\cite{wu2018blockdrop} and BranchyNet~\cite{teerapittayanon2016branchynet}. First two AdNNs follow conditional-skipping mechanism, while, BranchyNet is an early-termination model.
 In the following subsections, we will discuss the architecture of these two models.

\begin{comment}
  In SkipNet \cite{wang2018skipnet}, a shallow CNN or RNN network is used as gate and is placed in between different residual blocks of ResNet. If the gate output is less than 0.5 then the next residual block is not executed (or the block is `skipped'). 
  SACT \cite{figurnov2017spatially} and `early exit policy' \cite{bolukbasi2017adaptive} are of second type.
  SACT uses shallow convolution layer and average pooling to create a halting score for each spatial position at the output of a ResNet layer. For a residual block, The halting scores are added after each layer and when the sum reaches 1, then the spatial position is not calculated for next layers in the block (thus early termination). `Early exit policy' is used to train a CNN such that the policy determines if next layer should be executed or current output is sent to a simple classifier to get an result, thus breaking the network. In all three examples, changing the condition outputs can result in increase or decrease in number of computations, resulting change in inference time. For the first example it is gate output, for second it is summation of halting scores, and for the third it is confidence score. 
\end{comment}





\subsection{Conditional-skipping Architecture}
SkipNet is a gating-based AdNN which selects residual blocks based on gate outputs.
In SkipNet, gates are positioned in between two residual blocks. \footnote{Residual block consists of multiple layers whose output is determined by adding the output of the last layer and input to the block.}
To make a decision about skipping a block, at first, the input feature map ($X_{i}$) of the block is sent to the corresponding $i^{th}$ gate. Then, global average pooling and linear projection are applied on $X_{i}$.
This linearly projected input is fed to a Long Short Term Memory \cite{hochreiter1997long} (LSTM) with hidden unit of size ten. 
The LSTM output is changed to a one-dimensional vector, which is further sent for 2D convolution followed by a sigmoid function. The function output decides the final gate decision. If the output of the sigmoid function is greater than 0.5, then the corresponding block is not skipped. That block is termed as an \textit{active block}. If a block is skipped, the block input is passed to the next active block.
Each gate output has a dependency on all previous gate outputs (based on previous cell state and output of LSTM). 


The other conditional-skipping architecture, BlockDrop, uses a single policy network instead of gates to select the required residual blocks of a ResNet model. Policy Network is a simple residual network (ResNet-8) which is configured before the first block of the main ResNet architecture. At first, a trained ResNet is used to train the policy network using associative reinforcement learning. During inference, the trained policy network generates a binary policy vector, which represents the actions to keep or drop
a block in the pretrained ResNet. 


\subsection{Early-termination Architecture}

BranchyNet is an early-termination AdNN which uses exit points within a traditional DNN. Each exit point has few additional layers to create the output layer of a classifier. In the time of inference, each exit point tests for the confidence of the output. If the confidence score for an input for a certain exit point is high, \textit{i.e.}, the output entropy of an exit point is lesser than a certain threshold, the sample is exited and returns a predicted label
early.

Distributed Deep Neural Network (DDNN) \cite{teerapittayanon2017distributed} uses the energy-saving mechanism of BranchyNet to decrease inference time in edge devices. DDNN uses two different Neural Networks, one located in an edge device and another deployed in the cloud. If the local DNN fails to provide a prediction with high confidence, the input is sent to the cloud, whose network is more sophisticated, \textit{i.e.}, has more layers. DDNN can be extended to a system with multiple edge devices, each containing various DNNs with the final classification is done by aggregating all the DNN outputs. For our experiments, we have used the DDNN model as a stand-in for the BranchyNet paradigm.

\begin{comment}
For a residual block, SACT examines each position of the block input and decides if that position is needed to be processed in the next layer within the block. \footnote{Input to a residual block can be represented as a multidimensional matrix. In figure \ref{fig:SACT}, P0,P1,P2 and P3 are four positions of the block input.}
To make the decision, SACT applies Adaptive Computation Time (ACT) technique to each position of the input of the residual block. ACT technique computes a halting score for each position. To compute the halting score, a shallow convolution layer and average pooling is used. For a residual block, The halting score of each position is added after each layer. A position is called active if its cumulative halting score is less than one and inactive the cumulative halting score exceeds one. Inactive positions are not computed and the previous value of the inactive spatial positions are copied to be used as the current value. The evaluation of a block is stopped completely after all the positions become inactive. Ponder cost ($\rho$) of a position is the expressed as summation of number of residual units for which the position is active and the remainder value of the cumulative halting score after exceeding one. Generally, the ponder cost is averaged across the spatial positions for a block. 


Figure~\ref{fig:SACT} represents working mechanism of SACT using a single block of residual units. Halting score of each position for each unit is shown in figure. Lighter green color represents that the position became inactive.
\end{comment}

%\Cong{Critical: need to convince reviewers that the three techniques considered are 1. representative in both category 2. other AdNN methods are just incrementally built upon these three 3. these three techniques can be applied to most base DNN models, thus generalizable.}

%\Cong{add 2.3 explaining three AdNN techniques can be applied to many base DNN models etc.}




==> eval.tex <==
\section{Evaluation}


 


\begin{figure}[h!]
	\centering
	\includegraphics[width=0.53\textwidth]{figures/Imgnet_skipnet_seaborn.png}

	\caption{Percentage of flops increased by four perturbations for SkipNet model classifying Imagenet dataset}
	
	\label{fig:evalimgskip}
\end{figure}

\begin{figure}[h!]
	\centering
	\includegraphics[width=0.53\textwidth]{figures/cifar_skipnet_seaborn.png}

	\caption{Percentage of flops increased by four perturbations for SkipNet model classifying CIFAR-10 dataset}
	
	\label{fig:evalcifskip}
\end{figure}


\begin{figure}[h!]
	\centering
	\includegraphics[width=0.53\textwidth]{figures/Imgnet_SACT_seaborn.png}

	\caption{Percentage of flops increased by two perturbations for SACT model classifying Imagenet dataset}
	
	\label{fig:evalimgsact}
\end{figure}

\begin{figure}[h!]
	\centering
	\includegraphics[width=0.53\textwidth]{figures/cifar_SACT_seaborn.png}

	\caption{Percentage of flops increased by two perturbations for SACT model classifying CIFAR-10 dataset}
	
	\label{fig:evalcifsact}
\end{figure}

\begin{figure}[h!]
	\centering
	\includegraphics[width=0.53\textwidth]{figures/eu_distance.png}
    \caption{Euclidean distances between generated and perturbed image}
	\label{fig:eu}
\end{figure}

\begin{figure}[h!]
	\centering
	\includegraphics[width=0.53\textwidth]{figures/edge_detect.png}
    \caption{Difference in edges between generated and perturbed images}
	\label{fig:edge}
\end{figure}

\begin{figure}[h!]
	\centering
	\includegraphics[width=0.53\textwidth]{figures/FFT.png}
    \caption{Euclidean distances between FFTs of generated and perturbed images}
	\label{fig:fft}
\end{figure}



\begin{figure}[h!]
	\centering
	\includegraphics[width=0.53\textwidth]{figures/cifar_cost3.png}
    \caption{CPU power consumption of the techniques for Cifar10 images}
	\label{fig:cifcost}
\end{figure}
\begin{figure}[h!]
	\centering
	\includegraphics[width=0.53\textwidth]{figures/imgnet_cost.png}
    \caption{CPU power consumption of the techniques for Imagenet images}
	\label{fig:imgnetcost}
\end{figure}

\begin{figure*}[h!]
	\centering
	\includegraphics[width=1.0\textwidth]{figures/imgnet.pdf}
    \caption{Effect of different attacks on Imagenet dataset images}
	\label{fig:distimgnet}
\end{figure*}




We investigate the four characteristics of our attacks in this section: 


\textbf{Effectiveness - How effective is our attack to increase the computations during model inference with our attack-generated images?} Here we discuss the number of FLOPs increased during the inference by our attacked images. 


\textbf{Quality -  What is the quality of the attack-generated images?} We discuss traditional computer vision metrices to analyze how the attack affects the generated images. 


\textbf{Efficiency - What is the cost of different attacks?} We discuss the cost of our attacks in terms of time and energy consumption.

\textbf{Transferability - Are these attacks transferable to different models?} We discuss if these attacks are transferable between similar or different types of AdNNs. 

\begin{comment}
\textit{RQ1. Does the number of computations increase during model inference with our attack-generated images?} Here we discuss the number of FLOPs increased during the inference by our attacked images. 

\textit{RQ2. What is the pixel value difference between original and attacked image and how different hyper-parameters affect the attacked image?} We discuss the average change in image pixels after attack using different distortion initialization and different number of iterations.

\textit{RQ3. What is the cost of different attacks?} We discuss the cost of our attacks in terms of time and energy consumption?

\textit{RQ4. What is the change in energy consumption change with attacked images? } We discuss the energy consumption in mJ to show how much energy is consumed during the inference of the attacked vs the original image.

\textit{RQ5.Are these attacks transferable to different models?} We discuss if these attacks are transferable between similar or different types of AdNNs.

\textit{RQ6. What is the pattern of intermediate outputs after attack?} We discuss about the changes in gate outputs or ponder costs after the attack.
\end{comment}



\subsection{Experimental Setup}
\label{subsec:setup}

\textbf{Datasets.} We evaluated our techniques on CIFAR-10 and Imagenet datasets for SkipNet and SACT models. The reason for selecting the specific datasets was to maintain consistency as both the models have been previously evaluated on the same datasets. 
 
\textbf{Models.} SkipNet and SACT models can be built using ResNet models. SkipNet uses a modified ResNet-110 model to classify CIFAR-10 images and a modified ResNet-101 model to classify Imagenet images. SkipNet models are trained using supervised learning. SACT uses a ResNet-32 model to classify CIFAR-10 iamges and a ResNet-101 model to classify Imagenet dataset. 

Table \ref{tab:qual} represents the parameters used by Static and Borderline attack for SkipNet and SACT. The Active Gate Threshold ($T$) is the minimum threshold set for minimum number of gates that needs to be active ($S$) after the attack.
 The Ponder Cost Threshold is the threshold for mean ponder cost in SACT. The number of iterations for the `SLSQP' algorithm is 10. Due to higher time consumption of 'SLSQP', we have used only 10 iterations. Tolerance is acceptable relative error in satisfying constraint. 
Table \ref{tab:compare} lists the parameters used in L2 attack. Due to lower cost of L2 attack, we can use 300 iterations for Imagenet and 1000 iterations for CIFAR-10 dataset. The constant ($c$) used here is static and kept high because we are more concerned about $f(x+\delta)$ than $\delta$ (equation \eqref{eq:2}.

\begin{comment}
For different RQs, we created separate set ups.

\textbf{Setup 1.} This setup is for RQ1. 
  

\textbf{Setup 2.}
This is for RQ2. We select 100 Cifar10 input images and perturbed images from the images used in setup 1 and perform quality measurement on them. 

\textbf{Setup 3.}
For RQ1 and RQ3, we select 100 Cifar10 input images from setup 1 and attack those images. We measure energy consumption of the attacks and inference both. For measuring energy consumption, we use Nvidia TX2 server. 

\textbf{Setup 4.} This set up is for RQ4. The selected 100 images in Setup 3 is used again.  For RQ4, we use another SkipNet model which is trained using reinforcement learning.

\end{comment}

\begin{table}[t]
		\scriptsize\center\caption{\label{tab:thres} Different selection parameters used for AdNNs} 
		\begin{tabular}{|@{\hskip1pt}l@{\hskip1pt}|@{\hskip1pt}r@{\hskip1pt}|@{\hskip1pt}r@{\hskip1pt}|@{\hskip1pt}r@{\hskip1pt}|r@{\hskip1pt}|}
			\hline &  \multicolumn{2}{|c|}{SkipNet}&  \multicolumn{2}{|c|}{SACT}\\\cline{2-5}
		Threshold&CIFAR-10&Imagenet&CIFAR-10&Imagenet\\
			%Params&Cifar10&Imagenet\\
			\hline\hline { $\rho$ Threshold for selection}&--&--&11.5&25\\
			{ Active gate threshold for selection}&36&24&--&--\\
			\hline
		\end{tabular}
	\end{table}


\begin{table}[t]
		\scriptsize\center\caption{\label{tab:qual} Different parameters used for Constraint-based technique} 
		\begin{tabular}{|@{\hskip1pt}l@{\hskip1pt}|@{\hskip1pt}r@{\hskip1pt}|@{\hskip1pt}r@{\hskip1pt}|@{\hskip1pt}r@{\hskip1pt}|r@{\hskip1pt}|}
			\hline &  \multicolumn{2}{|c|}{SkipNet}&  \multicolumn{2}{|c|}{SACT}\\\cline{2-5}
		Params&CIFAR-10&Imagenet&CIFAR-10&Imagenet\\
			%Params&Cifar10&Imagenet\\
			\hline\hline{ $T$ }&42&29&--&-=\\
			{ Iterations}&300&10&--&--\\
			{ Tolerance}&1e-06&1e-06&--&--\\
			
			\hline
		\end{tabular}
	\end{table}


\begin{table}[t]
	\scriptsize\center\caption{\label{tab:compare}  Different parameters used for ILFO } 
	\begin{tabular}{|@{\hskip1pt}l@{\hskip1pt}|@{\hskip1pt}r@{\hskip1pt}|@{\hskip1pt}r@{\hskip1pt}|@{\hskip1pt}r@{\hskip1pt}|r@{\hskip1pt}|}
		\hline &  \multicolumn{2}{|c|}{SkipNet}&  \multicolumn{2}{|c|}{SACT}\\\cline{2-5}
		Params&CIFAR-10&Imagenet&CIFAR-10&Imagenet\\\hline\hline
		Iteration &1000 & 300&1000&300\\
		Constant&100000&100000&100000&100000\\
		learning rate &0.01&0.01&0.01&0.01\\
		\hline
		\end{tabular}
\end{table}

\subsection{Experimental Results}





\subsubsection{Effectiveness}  
\begin{comment}
\textbf{RQ1. How effective is our attack to increase the computations during model inference with our attack-generated images?}
\end{comment}

We measure effectiveness of the attacks by measuring increase in FLOPs during inference of attacked images. For this purpose, we process all the images from CIFAR-10 dataset and choose the images with lower energy consumption. Similarly for Imagenet dataset, we choose 700 images with lower energy consumption. For both the models (SACT and SkipNet), we set a threshold to know if the image consumes low energy or not. For SkipNet, this threshold is dependent on number of active gates while threshold is relied on ponder cost ($\rho$) for SACT. As pre-processing, Imagenet images are converted into shape $224\times224\times3$.
We compare ILFO with other two other approaches (baseline and constraint-based) to measure effectiveness. For baseline, we have used random gaussian noise. We have used Constraint-based attacks only on conditional-skipping AdNN (SkipNet) because creating constraint-based technique for early-termination AdNN (SACT) is time and resource consuming. 


Figure \ref{fig:evalimgskip},\ref{fig:evalcifskip},\ref{fig:evalimgsact},\ref{fig:evalcifsact} represents the increase of flops in terms of percentage. We have used box plots to show our results. Box plots uses boxes and whiskers to explain the results. First quartile, median and third quartile of the results are represented by boxes and the whiskers go from each quartile to the minimum or maximum. Outlier points are shown as separate points.
ILFO attack has performed better than other approaches for all models and datasets. For Cifar10 dataset, ILFO has increased the FLOPs count 32.5 \% for SkipNet model and 45.75 \% for SACT model on average. Average increase in FLOPs for gaussian noise (7.33 \%) is better than constraint-based attack (5.44 \%) for SkipNet. Although, gaussian noise has decreased the FLOPs count for few instances (represented through outliers). For SACT, gaussian noise can increase the number of FLOPs by only 1.47 \% on average. 
For Imagenet dataset, average percentage of FLOPs count increased by ILFO is 28.72 \% for SACT model. Gaussian model decreases the FLOPs count 0.7 \% on average. For SkipNet Model, ILFO is able to increase 29.4 \% FLOPs. Constraint-based technique is comparatively more successful for Imagenet datasets than CIFAR10. The technique can increase 11.28 \% FLOPs on average.

Based on performance, ILFO is more effective on Cifar10 dataset than Imagenet dataset. Although, the scope of increasing computations is higher for Cifar10 dataset than Imagenet because AdNN's performance on Cifar10 dataset is better than Imagenet dataset (\textit{e.g.,} SkipNet can reduce computation for Imagenet dataset by 29.9 \% which lower than the reduction for Cifar10 dataset which is 50.4 \%). Other than that, it is noticeable that the range of increase in FLOPs for Cifar10 images is larger than the range for Imagenet images. Initialization of perturbation can be one of the reasons behind this. We use randomized initialization of perturbation and for few inputs the optimization can get stuck at a local minima. However, we can refer from the results that there are few number of inputs (represented as outliers) for which the increment of computation is low.



\begin{comment}
Although, the increase in flops for Imagenet dataset after attacking SkipNet model is between 20-25 \%, the scope of increment was not very high in many of the images. 

Although, for those cases, our result shows that model could only save 3-5 percent of FLOPs after attack. Borderline attack performs best after L2 increasing 5-15 percent FLOPs. In principle, SkipNet focuses on the main object of the image and makes blocks active based on that. It is interesting that changing only outer part of the image can increase the computation too. Static attack has not performed well in any of the scenarios. The reason for this can be the 'SLSQP' optimization function. This function focuses more on the minimization than the constraints, so there are quite a few instances where it fails the constraints.
\end{comment}







\subsubsection{Quality}  
\begin{comment}

\textbf{RQ2. What is the quality of the attack-generated images? }
\end{comment}
\begin{figure*}[h!]
	\centering
	\includegraphics[width=1.0\textwidth]{figures/cifarimgs.pdf}
    \caption{Effect of different attacks on CIFAR-10 dataset images. }
	\label{fig:distcifar}
\end{figure*}

While implementing ILFO, we have chosen a high constant value ($c$) which is used for balancing both part of the loss function in equation (\eqref{eq:2}). Higher $c$ means higher weightage on increasing computation than minimizing perturbation. Because of this reason, the pixel difference between original and ILFO generated image can be higher than constraint-based technique generated image. Although, our results show that ILFO has limited effect on the quality of the generated image. To measure quality, we select 100 attacked image by ILFO and  constraint-based technique. These attacked  images are generated by attacking SkipNet model and the images are taken from Imagnet dataset.

 To measure the quality of the attacks, we use two traditional computer-vision algorithms used by Jang et. al. \cite{jang2017objective} other than measuring euclidean distance of pixel values of original and generated image. The two traditional algorithms are - \textit{Canny Edge Detection and Fast Fourier Transform}. These two algorithms helps to find out the effect of attack on the features of the image.

Canny Edge Detection (CED) is a method to detect edges in an image. Pixels whose value is significantly different from their neighbours are called edges. We use edge detection as a metric to measure quality by analyzing the change in number of edges in the image after attack. Canny edge detection follows certain steps to detect edges. After reducing the noise from the image, CED calculates intensity gradients by convolving the image with predefined Sobel filters. We get the information of changes of values over pixels. Next, edge thinning is performed by suppressing the gradient and finally, strong edges (higher gradient value) are selected represent the edges of the image. 

Fourier Transform is used to convert signals from spatial or temporal domain to frequency domain. Fast Fourier Transform (FFT) is an algorithm to perform Fourier Transform with lower time complexity. Converted spatial frequency domain can be useful in giving useful information regarding image features.
Rough shape structure of the image generates low spatial frequency after FFT. High spatial frequency corresponds to detailed feature (sharp change of illumination and edges).

Figure \ref{fig:distimgnet} and \ref{fig:distcifar} shows few of the resultant images created after ILFO and constraint-based attacks. Among the resultant images, ILFO generated images has highest average change in pixels (figure \ref{fig:eu}).  From figure \ref{fig:distimgnet} and \ref{fig:distcifar}, we can notice that the resultant ILFO attacked images are like the original images but with high contrast. Constraint-based technique only modify the border of the image for which the euclidean distance between attacked and original images is lower. 

Instead of having difference in euclidean distance of pixels, the effect of both attacks on image feature is similar. We measure the difference in detected edges between original and attacked images (figure \ref{fig:edge}). The average change in number of edges is 616 for ILFO and 582 for constraint-based technique which are similar. Euclidean distance between generated FFTs also shows the difference in features in the images (figure \ref{fig:fft}). The difference in average distance for ILFO and constrain-based technique is 2. These results shows that images generated by ILFO attack doesn't change the quality of the image in a large manner.





\begin{comment}
Although different attacks increase FLOP computations, attacks would not be very effective if the resultant image is largely different than input image. Figure \ref{fig:distimgnet} and \ref{fig:distcifar} shows few of the resultant images created after attacks. Baseline attack produces the mostly affected images in terms of distortion. The images produced after borderline attack is also differentiable when original borderline of the image does not have a solid color. Static attack has not been very successful in terms of increasing computations, although, the generated images is very similar to the generated one. After L2 attack, the contrast of the image becomes higher.   

\end{comment}


\subsubsection{Cost}

Higher computational complexity of non-linear constraint-based optimization has been the reason behind formulating a loss function based attack. We differentiate two mentioned techniques (ILFO and constraint-based) depending on the per iteration cost. For similar time intervals, we measure the number of iterations performed by the techniques and power consumption during that period.  We select 10 Cifar10 and Imagenet images from the selected images during efficiency measurement experiments and attacked using ILFO and constraint-based technique for SkipNet model. We use powerstat to measure CPU power consumption during both attacks. All the other programs which are using the CPU were terminated.  The number of iterations used for both techniques is mentioned in table \ref{tab:qual}. We noticed that  attacks on the first image in the dataset are more time consuming than the attacks performed on later images. Because of this reason, we show the power consumption of both that attacks on third image. Figure \ref{fig:cifcost} and \ref{fig:imgnetcost} shows the power consumption per second for two techniques for one image.


 
 Results show that the power consumed by both attacks are in the range of 20-40 watts. the difference in time consumption is also within 200 seconds. The main difference is the number of iterations. With similar amount of time and power consumption, ILFO performs larger number of iterations (700 more for Cifar10 and 290 more for Imagenet) which eventually helps to generate more effective attacks. 
  


\begin{comment}
\begin{table}[t]
	\scriptsize\center\caption{\label{tab:cost}  Different parameters used for Modifued L2 } 
	\begin{tabular}{|@{\hskip1pt}l@{\hskip1pt}|@{\hskip1pt}r@{\hskip1pt}|@{\hskip1pt}r@{\hskip1pt}|@{\hskip1pt}r@{\hskip1pt}|r@{\hskip1pt}|}
		\hline &  \multicolumn{2}{|c|}{SkipNet}&  \multicolumn{2}{|c|}{SACT}\\\cline{2-5}
		Type&CIFAR-10&Imagenet&CIFAR-10&Imagenet\\\hline\hline
		Static  &1000 & 554&--&--\\
		Borderline&100000&675&--&--\\
		L2 &0.01&850&0.01&0.01\\
		\hline
		\end{tabular}
\end{table}
\textbf{RQ4. How much the attacked images will change if we increase the number of iterations}

Other than knowing the increase in FLOPs, we also investigated the change in energy consumption (in mJ) after our attacks. For measuring energy consumption, we have used nvidia TX2 server. We selected 100 images from CIFAR-10 dataset and attacked those images with our techniques. We measured energy consumption of classifying those images by two models before and after the attack. 


\textbf{RQ5. How much attacked images will change if we use different initialization?}

We test the transferribility of our attacks by using our attacked images in a similar models. We have used attacked images for SkipNet in SACT and vice-versa. We also used a differently trained SkipNet model (Hybrid RL) for this purpose. We select 100 images from CIFAR-10 dataset for this experiment.
\textbf{RQ4. How much energy consumption will change after using the attacked images?}

All of our attacks has been dependent of initialization of the distortion. Although, it is very important to know which of the attacks dependence on initialization is more. 
\end{comment}


\subsubsection{Transferability}
Due to different architecture and different type of training process, we measure the transferability of our attack in two ways. For traditional DNNs, an attack is transferable if the attacked input generated attacking one model is processed through another model and gets misclassified. For AdNNs, we define that an attack is transferable if the attacked image doesn't decrease computation while being processed through another model. We discuss two types of transferability. First, we discuss transferability of attack between different sized and similarly trained model. Second, we discuss transferability of attack between different sized and differently trained model.

We use three types of SkipNet model for this purpose. These are - (a) SkipNet model trained using Reinforcement Learning and ResNet-110 model, (b) SkipNet model trained using Supervised Learning and ResNet-110 model and (c) SkipNet model trained using Reinforcement Learning and ResNet-38 model.
200 selected images used for evaluating effectiveness is used for experiments.

\textbf{Transferability of attack between different sized and similarly trained model}: For this experiment, we select model (a) and model (c). 




%\textbf{RQ6. What is the pattern of intermediate outputs after attack?}



\begin{comment}
We evaluated our techniques on CIFAR-10 dataset for both SkipNet and SACT models and Imagenet dataset for SkipNet model. The reason for choosing these two datasets is that these models were evaluated used the same datasets to report models' performance. We have processed all the images from CIFAR-10 dataset and chose the images with lower energy consumption and for Imagenet, we chose 100 images with lower energy consumption. The term 'lower energy consumption' is dependent on a threshold which varies for different models. As discussed earlier, SkipNet and SACT both are modified versions of ResNet. SkipNet uses modified ResNet-110 model to classify CIFAR-10 and ResNet-101 model to classify Imagenet images. SACT used ResNet-32 to classify CIFAR-10 images. For ResNet-110, there are 54 residual blocks. We call an image has consumed lower energy if its inference make less than 54 blocks active. Similarly, for ResNet -101, the thesold is 24 out of 33 blocks. For SACT, the lower energy threthan shold is dependent on mean ponder cost. For ResNet-32, if an image's ponder cost is less 11.5, we consider it low energy consuming image. 
\begin{table}[t]
	\scriptsize\center\caption{\label{tab:compare2}  Performmance Eval } 
	\begin{tabular}{|@{\hskip1pt}l@{\hskip1pt}|@{\hskip1pt}r@{\hskip1pt}|@{\hskip1pt}r@{\hskip1pt}|@{\hskip1pt}r@{\hskip1pt}|r@{\hskip1pt}|}
		\hline &  \multicolumn{2}{|c|}{SkipNet}&  \multicolumn{2}{|c|}{SACT}\\\cline{2-5}
		Models&CIFAR-10&Imagenet&CIFAR-10\\\hline\hline
		L2 &30.97\% & 26.97\%&42.4\%\\
		Borderline&7.16\%&11.06\%\%&----\\
		Static &2.85\%&2.99\%&----\\
		\hline
		\end{tabular}
\end{table}

Table \ref{tab:compare2} represents the increase in FLOPs through our attacks in terms of percentage. We can see that L2 attack has outperformed other attacks.
SACT uses ResNet-32 to classify CIFAR-10 and ResNet-101 model to classify Imagenet dataset.
\end{comment}



==> intro_changed.tex <==
\section{Introduction}
Deep neural networks (DNNs) have enabled
impressive accuracy improvements over traditional machine learning techniques in a variety of tasks, such as visual object recognition, speech recognition, and machine
translation. 
% CNNs (Convolutional Neural Networks) are a type of DNN mostly used for image classifications. 
% However, the power of CNNs comes at a considerable cost, namely, the computational cost of applying the CNNs to the new examples. 
However, these accuracy improvements depend on the availability of exceptionally large computational resources that necessitate substantial energy consumption as well~\cite{strubell2019energy}.
% This cost, often called the test-time cost, has increased rapidly for many tasks with ever-growing demands for improved performance in state-of-the-art systems. 
The computations required for deep learning research doubles every few months, resulting in an
estimated 300,000x increase from 2012 to 2018~\cite{energy}.
The ResNet152 architecture \cite{he2016deep} with 152 layers, realizes a substantial 4.4\% accuracy
gain in top-5 performance over GoogLeNet\cite{szegedy2015going} on the large-scale ImageNet dataset but is about 14X slower at test-time. This increased test-time cost has become a problem especially in the cases where faster inference is required (\textit{e.g.} mobile apps). 
% Image recognition techniques is now being used in a large number of mobile applications. In many cases, higher inference time can be a big problem. 
For example, a visually impaired user may use an app based on DNNs for object detection. 
The prolonged response time of DNNs will cause fatal issues for the user relying on the app.

To address these problems, extensive research has been proposed and proposed models are called \textit{energy-saving models}. There have been two types of 
energy-saving models: On-Device Neural Networks (ODNN) and Adaptive Neural Networks (AdNN). 
ODNN models~\cite{iandola2016squeezenet,howard2017mobilenets,zhang2018shufflenet}  use lower dimensions of filters or change the dimension of input to the filters to decrease the number of computations, while AdNN dynamically deactivate a certain part of the model based on different inputs to reduce the number of computations.



\begin{comment}
inference time is different for different images based on `complexity' of the image \footnote{In that way, images which are `easier' to classify will use fewer parameters than other images}.  
\end{comment}
Attackers are motivated to attack the energy-saving models mentioned above because of damaging consequences. For example, SkipNet \cite{wang2018skipnet}, an AdNN model, can reduce 50 \% of floating-point operations in a ResNet model for the CIFAR-10 dataset. If an attack on the input can increase 35-40 \% of the reduced flops, the purpose of the SkipNet model would not be served. This type of decrease in performance will eventually jeopardize the reputation of the app or software which uses the energy-saving model. 


Investigating the robustness of these energy-saving models for energy consumption is needed to protect them from potential attacks.
 The robustness of a machine learning model can be defined as the stability of the model accuracy after adding some noise to input data \textit{i.e.,} a robust model's accuracy will not deteriorate against noisy inputs. We define a new term \textit{energy-robustness}, which is defined as the stability of the model's energy consumption after getting a perturbed input. 
 \begin{comment}
 For non energy-saving models, performance is evaluated by the prediction accuracy of the model. Although, the performance of an energy-saving model includes both reduction in energy consumption and prediction accuracy of a model.
 \end{comment}
% Adversarial Machine Learning techniques have been used to investigate the robustness of a model in terms of prediction accuracy. Traditional adversarial attacks add noise to the inputs to make the model prediction false. These traditional attack techniques use the relation between input and output to change the output. Although, those attacks are not relevant to investigate the energy robustness of the energy-saving models. 
Traditional adversarial machine learning techniques formulate their attacks based on the relation between input and output. 
However, energy robustness considers the relation between input and its corresponding energy consumption.
In section~\ref{sec:form}, we show that the attack formulation for energy robustness requires detailed knowledge about the model and needs to define the target values for different AdNNs.
Before this work, there has not been any technique which can investigate the energy-robustness of a model.  In this paper, we are motivated to investigate the robustness of the energy-saving models by generating perturbed images to increase the energy consumption of these models.
Specifically, we use AdNN as an example to perform such investigation. In our knowledge, this is the first attempt towards this direction.

However, attacking a model with respect to energy consumption is complicated because it is impossible to find a trail from input to energy consumption during inference. There are multiple systems (\textit{e.g.}, Nvidia TX2 server, FogNode, Raspberry Pi) which can measure the energy consumption of machine learning model inference. Although, the energy consumption measured using these systems is not dependent on only the model. The measurement is also dependent on system environment. This also makes impossible to find out the pattern in energy consumption in different images. If an image inference consumes less amount of energy then it is difficult to conclude if it is because of the input or the system environment.

 Due to the difficulty to relate input and energy consumption, we attack the energy-saving models by increasing the number of computations during inference. For traditional DNNs and ODNNs, number of computations during inference is constant \textit{i.e.,} we can not relate the number of computations with input. Although, AdNNs change the number of computations based on intermediate layer-wise outputs. Creating a relation between input and intermediate outputs relates input and number of computations. 
 In this paper, we have explored the relation between inputs and intermediate outputs of AdNNs and attack these models.
 


%Before proposing new techniques to investigate robustness about energy consumption, we would like to %address why traditional black box attacks can not be used to increase energy consumption of a model.
\begin{comment}
However, attacking a model with respect to energy consumption is complicated. For traditional DNNs (\textit{e.g.,} non-energy saving DNNs), the number of parameters to be used for inference is constant. The number of used parameters in a model is proportional to the energy consumption in a model. Changing  inputs can not change the number of used parameters in a traditional DNN so it can not change the energy consumption also.
%When the number of parameters is constant, the energy consumption can change only due to framework and %hardware specifications (\textit{e.g.,}cache memory, processor speed).  
Our preliminary results support this fact by showing that, for a traditional DNN model, the range of model's energy consumption is very small for different inputs (Section \ref{sec:prelim}). 
A model's inference energy consumption can be reliant on input if the number of used parameters for the model is dependent of model-generated values.
In that scenario, we can change energy consumption using input if we can establish a relation between input and those model-generated values.
Traditional gradient based attack techniques \cite{papernot2016limitations,carlini2017towards,goodfellow2014explaining} exploit the relation between input and output to attack the model. We can use similar gradient based techniques to attack an energy-saving model based on the relation between model-generated values and input.
 AdNN models deactivate a certain part of the model based on input and in this way number of used parameters in AdNN is dynamic. AdNNs use intermediate layer-wise outputs to deactivate certain part.
In this paper, We have explored the relation between inputs and intermediate outputs of AdNNs and attack these models.

\end{comment}
\begin{comment}
The energy consumption during inference can be associated with the number of floating point operations (FLOPs) and FLOPs are not directly related to the output. For example, ResNet and AlexNet can both successfully classify an image but ResNet consumes significantly more amount of energy than AlexNet during inference.
Traditional attacks like \cite{papernot2016limitations,carlini2017towards,goodfellow2014explaining} has been designed to change the output of the sample with minor changes in the input sample using the gradient of generated output with respect to the input. While this gradient can be useful to change the output, it is not related to the energy consumption of the classification process.  Because of this reason, traditional attacks can not be applied in terms of increasing energy consumption. To increase energy consumption in an energy-saving model (\textit{e.g.,} AdNNs), intermediate layer wise outputs are most important because these intermediate outputs are used to decrease the number of FLOPs in AdNN. 
\end{comment}

%AdNN generates these intermediate outputs based
 
   We are proposing ILFO (\textbf{I}ntermediate Output Based \textbf{L}oss \textbf{F}unction \textbf{O}ptimization) to attack AdNNs. Using the gradient between intermediate outputs and inputs, we create a loss function and optimize that function. Function optimization changes the intermediate inputs which activates the deactivated part of the AdNN model increasing number of computations. In this paper, after giving a brief idea about the different AdNN models (section \ref{sec:back}), we have formulated the idea of ILFO (section \ref{sec:form}). In section \ref{sec:approach}, we have explained the approach ILFO. We have evaluated ILFO based on four characteristics - effectiveness, quality, and efficiency. Our results show that ILFO could increase the Floating-Point Operations (FLOPs) during inference of the image up to 100 \% . 
   
   
   

\begin{comment}
A model will be robust in terms of energy consumption if slightly altering input does not affect the energy consumption of a model.There has been multiple ways to measure energy of a model. Zhang et. al. \cite{zhang2018pcamp}, measured energy of different models on Macbook, Fognode and Jetson TX2 server in terms of Joule(J). The authors also found out from the experiments that latency or test time is directly proportional to the energy. On the other side, test time depends on the floating point operations (FLOPs). Traditional CNN models are more robust in terms of energy consumption because they perform same number of FLOPs on every image. The other models, like AdNN, compute different number of FLOPs for different images. The AdNN models can be robust only if FLOP count is not changed significantly with slight alteration to the input.

 AdNNs has been proposed to overcome the problem of higher test-time. It has been observed that some of the images are easier to get classified while it is very tough to classify some and AdNNs uses that observation to build the network. There are mainly two types of Adaptive Neural Networks. First type is \textbf{Single CNN AdNN}, a traditional CNN model is structurally modified to save inference time. Second is \textbf{Multiple CNN AdNN}, multiple traditional CNNs are connected with a network and image is sent to any of the CNNs for inference based on image complexity. Although these techniques are new, still these techniques have been able to decrease test-time with a little decrease in accuracy.


 On the other side, adversarial machine learning techniques have been very significant exploring the vulnerabilities of machine learning models. Adversarial techniques or attacks use malicious inputs to `fool' a machine learning model. Fooling a machine learning model means perturbing the input features in such a way that the model makes a false prediction. Although, there has not been much exploration about attacking machine learning models in terms of energy. There has been multiple ways to measure energy of a model. Zhang et. al. \cite{zhang2018pcamp}, measured energy of different models on Macbook, Fognode and Jetson TX2 server in terms of Joule(J). The authors also found out from the experiments that latency or test time is directly proportional to the energy. We measured energy of different CNN models (ResNet, GoogLeNet and Alexnet) on Jetson TX2 server. While we found out that energy consumption is directly proportional to number of layers (or FLOPs), we could not directly map the energy consumption recorded to test images because a single image consumes different energy while measuring at different times. This is the reason it is difficult to adversarially attack traditional CNN models in terms of energy. We have tried to explore a new type of CNNs in this paper, \textit{i.e.,} Adaptive Neural Networks.
 
\end{comment}




 

Our paper makes the following contributions:

(i) This is the first work investigating the robustness of neural networks in terms of energy consumption.

(ii) ILFO could increase the FLOPs during inference up to 100 \%.

(iii) ILFO tries to formulate a generic approach towards attacking all types of AdNNs.
 

 
 












==> new_approach.tex <==
\section{Problem Formulation}
\label{sec:form}
\begin{comment}
Time consumption in Machine Learning is a relevant topic because the current deep learning models consume significant amount of time for inference. Decreasing or increasing inference time based on input for the popular deep learning models (mainly CNNs) is a new and relevant topic of research. While formulating an algorithm to change inference time of CNNs will be an important research finding, our research findings suggested that for different inputs, the inference time of popular CNNs (\textit{e.g.,} ResNet, GoogLeNet) does not change significantly. Adaptive Neural Networks were proposed to overcome this shortcoming of traditional CNNs. It has been observed that some of the images are easier to get classified while it is very tough to classify some. Adaptive Neural Networks uses this observation to create the network. 

Adaptive Neural Networks can be very useful in mobile apps. Image recognition is being used in large number of mobile apps.From using face recognition to helping visually impaired people by object recognition, the number of applications is very high. These mobile apps can not always use object recognition architectures like ResNet and GoogLeNet because these architectures take significant amount of time for inference and mobile apps can become slow. For example, a visually impaired person is using an app for object detection while crossing a road. If the response time is slow then the person will face difficulty. Adaptive Neural Networks will be very useful in this scenario. While adaptive neural networks can be very effective, those are can be vulnerable for adversarial attacks. In future sections, we have discussed how to generate an adversarial image input for adaptive neural networks such that the inference time of the network increases.



There are mainly two type of Adaptive Neural Networks. First, one CNN is selected and then the network is modified to save inference time. Second,multiple CNNs are selected and image is sent to any of the CNNs for inference based on image complexity. We have focused on the first type.

\end{comment}

Our objective is to attack AdNNs by creating modified inputs which will increase the energy consumption of AdNNs during inference. The attack should concentrate on two factors. First, the attacked image should consume more energy during inference. Second, the attacked image and original image can not be differentiated. For every AdNN, we define two states of the intermediate outputs - desirable state ($des$) and current state ($cur$). $des$ defines the state of intermediate outputs for which computations during inference will be maximum. $cur$ is the current state of intermediate outputs. For an input $x$, we search for the perturbation $\delta$ for which $f(x+\delta)$ is minimum. $f(x+\delta)$ represents the difference between $des$ and $cur$. The optimization function can be represented as,
\begin{gather}\label{eq:2}
minimize(\delta+c \cdot f(x+\delta)) \mbox{ such that, }(x+\delta) \in [0,1]^n\
\end{gather}
The $c$ is a suitably chosen constant value and $c>0$. Our approach formulates the attack for each AdNN and converts the attack in the form of equation \eqref{eq:2}.
Based on the working mechanism of the two models discussed in section \ref{sec:back}, we have formulated our attacks.


\subsection{Attacking Early-termination AdNN}

Figure \ref{fig:SACT} represents the working mechanism of a residual block in SACT. SACT calculates halting scores as intermediate outputs. Within a residual block, these halting scores are calculated for each position after each layer. In SACT, the condition is the cumulative halting score for a position within a block should be less than 1 to make the position inactive. In the figure, Deep green positions are active while light green positions are inactive. To increase the energy consumption in SACT, 
the principle approach should be minimizing the halting scores generated at each layer for each position. In that way, the position will be active for more number of layers. Formulating an attack based on halting score would require a large number of intermediate outputs upon which the computations will depend. \footnote{For each position of each layer input, halting scores are calculated.}
 Because of this reason, we would use ponder cost of each position. As defined earlier in section \ref{sec:back}, ponder cost ($\rho$) of a position is the summation of the number of residual units(layers) for which the position is active and the remainder value of the cumulative halting score after exceeding 1. Ponder cost map will store the ponder costs of all input positions for a residual block. 
In figure \ref{fig:SACT}, P0, P1, P2, P3 are four spatial positions, $\rho_0$, $\rho_1$, $\rho_2$, $\rho_3$ are the ponder costs of those four positions . The value of $\rho_0$ will be 1 because P0 is active for only one layer and there is no remainder of the cumulative halting score after exceeding 1. Similarly for $\rho_2$, the value will be 3.1 because P2 is active for 3 layers and the remainder is 0.1 (0.2+0.1+0.8-1.0=0.1). $\rho_1$ and $\rho_3$ will be 1.0 and 2.1 respectively.  Increasing ponder cost of each position, will increase the computation of each position. 

Creating an attack directly using ponder cost maps can be complex because ponder cost maps are multi-dimensional arrays which the dimensions can be different for depending on residual blocks. Using resizing and addition, we create a smaller size 2D array to represent ponder costs. Resizing is a step that is not performed while attacking a traditional DNN. 
As shown in Figure 4, $\rho 
_{arr}$ represents the generated array  and $\rho _{arr}[i][j]$ represents ponder cost in the $i^{th}$ row and $j^{th}$ column of the $\rho _{arr}$. 
To represent our formulated attack using \eqref{eq:2}, we need to define the ideal behavior of $\rho _{arr}$.
We want each ponder cost of the $\rho _{arr}$ to get increased and reach a certain predefined threshold represented by $\rho _T$. With each iteration, Perturbation can be added to the input such that, each ponder cost in $\rho _{arr}$ exceeds $\rho _T$ at the end of the iterations. Before inserting perturbation at an iteration, if $\rho _{arr}[i][j]$ has exceeded $\rho _T$, then the value at $\rho _{arr}[i][j]$ should remain the same after adding perturbation. Otherwise, value at $\rho _{arr}[i][j]$ should increase.
We represent the principle for each iteration in the following way.








\begin{equation} \label{eq:new}
    \rho _{arr}[i][j](x+\delta'+\Delta)=
    \begin{cases}
      \rho _{arr}[i][j](x+\delta'), \text{if}\\ \rho _{arr}[i][j](x+\delta') >=\rho _T \\
      \rho _{arr}[i][j](x+\delta')+\Delta\rho,\text{otherwise}
    \end{cases}
 \end{equation}
 
 Here, $\delta'$ total added perturbation before iteration,  $\Delta$ is the perturbation being added at iteration, $x$ is input, $\Delta\rho$ is the value added at $\rho _{arr}[i][j]$. Figure \ref{fig:attackSACT} represent the approach through example.
 
 We can represent this maximization problem in the equation \eqref{eq:new} using equation \eqref{eq:2}. For this problem, the current state ($cur$) can be represented by $\rho _{arr}$. For desirable state ($des$), we define another array $\rho _{max}$ with the same dimension as $\rho _{arr}$ where,
 $\sum_{i=0}^{R}\sum_{j=0}^{C} \rho _{max}[i][j]=\rho _T$. $R$ and $C$ represent the dimension of $\rho _{max}$. Minimizing the difference between $des$ and $cur$ would increase the number of computations. We represent loss function $f(x+\delta)$ as,
 
 $f(x+\delta)=\sum_{i=0}^{R}\sum_{j=0}^{C} max(\rho _{max}[i][j]-\rho _{arr}[i][j],0)$
 
 The $max$ function ensures that any value in $\rho _{arr}$ does not get decreased. We can represent the formulation problem using equation \eqref{eq:2} replacing $f(x+\delta)$.
 
 
 
 



 
\begin{figure}[t]%
	\centering
	\includegraphics[width=0.5\textwidth]{figures/SACT_2.pdf}

	\caption{Working mechanism of a residual block in SACT}
	
	\label{fig:SACT}
\end{figure}

\begin{figure}[t]%
	\centering
	\includegraphics[width=0.53\textwidth]{figures/sact_attackalgo.pdf}

	\caption{Attack mechanism for SACT. $\rho _{arr}$ values less than $\rho _T$ (37 in the example) tries to exceed $\rho _T$ after each iteration. Values greater than $\rho _T$ tries to remain same.}
	\label{fig:attackSACT}
	
\end{figure}


\subsection{Attacking Conditional-skipping AdNN}


\begin{figure}[t]%
	\centering
	\includegraphics[width=0.52\textwidth]{figures/skipnet_2.pdf}

	\caption{Working mechanism of SkipNet. $B_0,B_1...,B_N$ represents residual blocks.}
	
	\label{fig:example}
\end{figure}


Figure \ref{fig:example} represents working mechanism of a SkipNet model containing $N+1$ residual blocks and gates corresponding to the blocks. A block becomes active if corresponding gate output exceeds threshold $G_T$. In figure \ref{fig:example}, the gates are represented as $G_i$ where $i\in[0,N]$. $\alpha_i(x)$ is a boolean variable which becomes true when $Output(G_i)>=G_T$, where x is the input image and $G_T$ is the threshold value to make a gate active.
$\alpha_i(x) = Output(G_i)>=G_T$

In the model shown in the figure \ref{fig:example}, $\alpha_0(x)$ and $\alpha_N(x)$ are $True$ while $\alpha_1(x)$ is $False$. All the residual blocks will be active if $\alpha_0(x) \land \alpha_1(x)..... \land \alpha_N(x)$ is true. If the input image is $x$ and attacked image is $x+\delta$, then we can formulate the attack in two ways. The first way is to represent it as an optimization problem with constraints. 


\begin{gather}\label{eq:1}
minimize(\delta), \\
\begin{aligned}
\mbox{such that, } \alpha_0(x+\delta) \land \alpha_1(x+\delta)..... \land \alpha_N(x+\delta)=True
\end{aligned}\notag
\end{gather}


Although equation \eqref{eq:1} can fulfil our objective, non-linearity of the constraints can increase the complexity. The other way is to represent the attack using equation \eqref{eq:2}. We define $G _{arr}$, an 1D array representing the gate outputs. $G _{arr}[i]$ represents $i^{th}$ gate output. In an iterative way we add perturbation to the input $x$ such that the gate outputs, which have a value lower than 0.5, reach 0.5 and other outputs remain same. The representation of the principle is,

\begin{equation} \label{eq:new2}
    G _{arr}[i](x+\delta'+\Delta)=
    \begin{cases}
      G _{arr}[i](x+\delta'), \text{if}\ G _{arr}[i](x+\delta')\\ >=G_T \\
      G _{arr}[i](x+\delta')+\Delta g,\text{otherwise}
    \end{cases}
 \end{equation}
 
 \begin{figure}[t]%
	\centering
	\includegraphics[width=0.52\textwidth]{figures/skipnet_attackalgo.pdf}

	\caption{Attack mechanism for SkipNet. $G_{arr}$ values less than $G_T$ tries to exceed $G_T$ after each iteration. Values greater than $G_T$ tries to remain same. $G_T$ is 0.5 in this example}
	\label{fig:attackskip}
	
\end{figure}

Here, $\delta'$ total added perturbation before iteration,  $\Delta$ is the perturbation being added at iteration,  $\Delta g$ is the value added at $G _{arr}[i]$. Figure \ref{fig:attackskip} represent the principle through example.

To formulate the attack like equation \eqref{eq:1}, we define $G _{arr}[i]$ as current state ($cur$). We define array $G _{max}$ with same dimension as $G _{arr}$. $G _{max}$ can be represented as  
$G _{max}[i]=\sum_{i=0}^{N}G_T$ and we define $G _{max}$ as $des$. We define loss function $f(x+\delta)$ as,
$f(x+\delta)=\sum_{i=0}^{N}max(0, G _{max}[i]-G _{arr}[i])$
By replacing loss function, we formulate the attack using equation \eqref{eq:2}.

\begin{comment}
We have formulised equation \eqref{eq:1} in a second way by removing the constraints and representing the constraints as a part of the optimization process. For this purpose, we define a loss function and optimize the function along with distortion. Carlini et. al. \cite{carlini2017towards} and Szegedy et. al. \cite{szegedy2013intriguing} have used loss function optimization in formulating traditional white box adversarial attack. Those loss functions are designed to optimize a loss function which helps to change the output label.
 For example, Szegedy et. al. have used cross entropy between desired output label and current output label as loss function. For AdNNs, we need to modify the loss function by incorporating intermediate outputs.
 With respect to intermediate outputs, we define two states - desirable state ($des$) and current state ($cur$). $des$ represents what the intermediate outputs would look like if we want to make number of computations maximum. For SkipNet, we would like to make all gate outputs greater than or equal to 0.5. In this case, 
$des$ would be a list where all values are 0.5 and size of the list will be same as the number of gates.  $cur$ represents the current gate output values. The loss function $f(x+\delta)$ is the difference between $des$ and $cur$ values where value in $cur$ does not exceed the $des$ value.

$f(x+\delta)=\sum_{i=0}^{N}max(0, des_i-cur_i)$

where, the number of gates is $N+1$.
%$=loss_{des,cur}(x+\delta)$ is the difference between $des$ and $cur$. 
We would try to minimize the function $f(x+\delta)$ along with the distortion and also make sure that generated pixel values should be within the limit 0 and 1. 


let's assume set A = $\{ \alpha_1, \alpha_2,...,\alpha_k \}$ where k is the number of gates and set $B \subseteq A$. $C$ is the cardinality of set $B$. Instead of checking if all $\alpha$ values are true , we will try to find a set $B$ where minimum number of $\alpha$ s are false.


\begin{gather}\label{eq:2}
minimize(\delta+c \cdot f(x+\delta))\\
\intertext{such that,} 
\begin{aligned}
(x+\delta) \in [0,1]^n
\end{aligned}\notag
\end{gather}

The $c$ is a suitably chosen constant value and $c>0$.
\end{comment}
\begin{comment}Our objective is the maximize the number of $\alpha$s which are true. For formulising the problem, let's assume set A = $\{ \alpha_1, \alpha_2,...,\alpha_k \}$ where k is the number of gates and set $B \subseteq A$. The objective can be represented as, 

$maximize(C)$ s.t., $\alpha_i \lor \alpha_{i+1} \lor ... \alpha_{i+C} = True$ where $\alpha_i, \alpha_{i+1} , ... \alpha_{i+C} \in B$ and $C$ is $|B|$. 



\subsection{Difference between attacking traditional DNN and AdNN}
\label{subsec:diff}

There are two main differences between attack formulation for AdNN and traditional DNNs. First, defining how the intermediate outputs should be changed or setting a `target' for intermediate outputs. Second, defining the `success' of the attack.
The main task to attack AdNN is to find desirable ($des$) and current ($cur$) states. For traditional white box attacks, these states can be defined using output layers. For traditional white box attacks, $des$ is the target output and $cur$ is the current output of the model. In the case of AdNNs, the $des$ and $cur$ states are dependent on the architecture of AdNNs. For this reason, detailed knowledge of the architecture of AdNN is required to attack AdNN.

Knowing the architecture of AdNN may not be enough to define $des$ and $cur$ because of the number of intermediate outputs responsible to increase computations. Traditional attacks uses single output values or a fixed size list of output values (\textit{e.g.,} logit values) to create the attack. For AdNNs, attack is never based on a single intermediate output value. In some cases, the number of intermediate output values can be very large and resizing of the number of intermediate outputs is needed to define $cur$ state \footnote{For example, SACT has different ponder cost values for each position in the feature map for each residual block. We use resizing and adding to create a matrix of ponder cost values which has same dimension as the input.}. Because of these reasons, pre-defining is an important step is attacking AdNN which is not required in attacking DNNs.

Like desirable state, we need to define the success of attacking an AdNN. For traditional attacks, the term `success' is binary. If an attack can change the output label of the classifier is termed as successful attack. Otherwise, it is unsuccessful. In that scenario, the output probabilities of the model does not come into consideration. Because of this reason, multiple techniques has been been successful and comparison between two attack techniques is mainly based on attack efficiency, output quality and cost of attack.
For AdNN, we define 
the success of an attack on increase in computations during inference after attack, \textit{i.e.,} the success of an attack is not binary. While comparing two attack techniques for AdNN, increase in computations would get preference over other metrics like output quality. While implementing the algorithm, we give preference on increasing computations than minimizing perturbations.


 \end{comment}


\section{Approach}
\label{sec:approach}

We propose ILFO based on the equation \eqref{eq:2}. Later in the section, we also discuss another technique based on equation \eqref{eq:1}. We call this technique constraint-based technique because the increase in energy consumption is represented by non-linear constraints. The usage of constraint-based technique is limited (Only conditional-skipping AdNNs here) and does not perform well in compare to ILFO.





\begin{comment}
$K$ are the pixels in image borderline,
$I$ is image input, $I^\prime$ is distorted image input represented by,

$I^\prime = merge_{l \notin K,k \in K}(I[l],V[k])$. 

\textbf{Static Perturbation Attack.} In this attack, we add a static perturbation to every pixel of the image. Figure \ref{fig:approachstatic} describes the flow of this technique. This attack uses SLSQP as optimization function which can find a local minima and for complicated non linear functions like ResNet, the probability of stucking in to a local minima is high. To handle this problem, we generate an initial distortion. We randomly generate 100 values for distortion and select the value which generates highest energy increase and has the lowest absolute value. Then the constraints are created based on the weighted sum technique or mean ponder cost mentioned earlier. A function returning the absolute value of the distortion is the function the algorithm will try to minimize. Finally, using the initial value, constraints and function, optimization algorithm is called.







\textbf{Borderline Perturbation Attack.} Based on the the second approach mentioned earlier, we tried to change up to ten pixels in the image but the number of computations in the SkipNet did not change significantly. Instead of that, we distorted relatively more number of pixels but all the pixels are in image borderline. In this way, We distorted only 3 percent of image pixels without affecting the main object in the image. 

Figure \ref{fig:approachborder} represents the flow of the attack. Initialization is an important step in this attack also as the static perturbation attack. In this attack, initial values of borderline pixels are evaluated instead of distortion. The constraint formation in this attack is same as the static perturbation attack. Borderline attack does not have any single perturbation, and because of this reason the optimization function tries minimize the difference between new borderline pixel values and original values. Finally, optimization function is called.




Minimization function will be different than static perturbation attack although constraints will be same. For SkipNet, the optimization is,


For SACT, the function will be,
$minimize(\sum_{k \in K}abs(I[k]-V[k]))$  $s.t.$  $(MPC(I^\prime) > T_P)$ 

Where, $MPC$ is a method that returns mean ponder cost of SACT and $T_P$ is threshold for ponder cost.

This approach does not distort all the image pixels but the pixels within a list $K$. $merge$ function merges the original image and distorted pixels to create new image $I^\prime$.



\begin{figure}[t]%
	\centering
	\includegraphics[width=0.53\textwidth]{figures/Approach1.pdf}

	\caption{Steps of Borderline Perturbation Attack}
	
	\label{fig:approachborder}
\end{figure}
\end{comment}

\subsection{ILFO}
\begin{comment}
Constraint-based perturbation attacks fulfil the requirement of increase in computation, they have some limitations. First, both attacks have a high dependency on initial values. It has been observed that with different initial values, the results could be different because the optimization can find a local minima. Second, having too many unknowns can slow constraint-based techniques  down. If we want to find different distortion for each pixel, constraint-based techniques would have large number of unknown values (224*224 for an Imagenet dataset image) making the algorithm very slow. Third, constraint-based techniques is time consuming. One of the reasons of these limitations are the non-linearity of the constraints. 
For this reason, we removed the constraints and formulated an attack which can incorporate both distortion and energy consumption as the optimization problem. we call this type of attacks as loss-based attacks.




For loss based attacks, we first define the loss function. With respect to intermediate outputs, we define two states - desirable state ($des$) and current state ($cur$). $des$ represents what the intermediate outputs would look like if we want to make energy consumption very high. For example, we would like to make all gate outputs greater than or equal to 0.5 in SkipNet. In that case, 
$des$ would be a list where all values are 0.5 and size of the list will be same as the number of gates. For SACT, $des$ will be a very high ponder cost value \footnote{A mean ponder cost is considered high when value is greater than 24.9}. $cur$ represents the current intermediate output values. Loss function $f(I')=loss_{des,cur}(I')$ is the difference between $des$ and $cur$ where $I'$ is the distorted image. We would try to minimize the function $f(I')$ along with the distortion. 
We can define the minimization problem as,

$minimize$ $D(I,I')+c \cdot f(I')$ 

such that $I' \epsilon [0,1]^n$ , where I is the input image, D is the function which measures distance between images and $c > 0$ is a suitably chosen constant. We have considered that all pixel values are between 0 and 1 after normalization.

Constraint-based techniques use non-linear constraints which make the algorithm time-consuming. Because of this reason, we create loss based technique based on equation 2 \eqref{eq:2}. To make sure that generated image pixels does not exceed the limit, we use $tanh$ function. $tanh$ function can convert a value to a new value within the range -1 and 1. We use this property of $tanh$ function and send the distorted values to a $tanh$ function.


The distance measure we have used is L2 distance which implies euclidean distance between pixel values two images. The measure has also been used by Carlini et. al. \cite{carlini2017towards}. We name this attack \textit{L2 attack}.

\end{comment}

ILFO is an iterative technique which generates the best possible perturbation for which the loss function value (mentioned in \ref{sec:form}) will be minimum. ILFO needs a pre-defining stage before the procedure which helps to formulate the loss function.
Figure \ref{fig:approachILFO} represents the pre-defining stage and the overview of ILFO. Sub-figure (a) represents the pre-defining stage. In this stage, desirable ($des$) and current ($cur$) states are defined based on the intermediate outputs of AdNN and a single or multi-dimensional array is used to represent the states. The loss function is defined based on the difference of these two states.
Sub-figure (b) represents overview of ILFO. ILFO takes image as input and generates the perturbed image using optimizing the loss function which was defined on pre-defining stage. 

%ILFO uses fixed number of iterations and adam optimizer is used for optimization. To measure the %distance between two images, we use euclidean distance. 

After adding perturbation to the image, it is important to make sure that the generated values are within the maximum and minimum limit for the inference. We use $tanh$ function to fulfil this purpose. The $tanh$ function can convert a value to a new value within the range -1 and 1. We use this property of $tanh$ function and send the distorted image values to a $tanh$ function. 
The optimization function for ILFO is a modified version of equation \eqref{eq:2}. 



\begin{figure}[t]%
	\centering
	\includegraphics[width=0.52\textwidth]{figures/ILFO_1.pdf}
	\caption{(a). Pre-defining the loss function. (b). Overview of ILFO Technique}
	
	\label{fig:approachILFO}
\end{figure}

\begin{gather}\label{eq:5}
\begin{aligned}
minimize ||\frac{1}{2} \cdot (tanh(w) + 1)-I||_2^2 +\\
c \cdot f(\frac{1}{2} \cdot (tanh(w) + 1))
\end{aligned}
\intertext{Where, $w$ is the generated perturbation.} \notag
\end{gather}

\begin{algorithm}[h]
\scriptsize
%\footnotesize
  %\DontPrintSemicolon
  %\SetAlFnt{\scriptsize\scriptfont}
  %\SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
  %\SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
  \SetKwInOut{Input}{Inputs}\SetKwInOut{Output}{Outputs}
  %\SetKwInOut{Input}{Inputs}\SetKwInOut{Output}{Outputs}
  \caption{ILFO Technique}\label{alg:L2}
  %\tcc{\textbf{forward crawling from a state}}
  \Input{$input\_image$ \\}
  \Output{$final\_attacked\_image$\\
  }
  \BlankLine
  \Begin{
    $Initialize$ $modifier, min\_loss,best\_solution,des$\\
    $T=number\_of\_iterations$\\
    $iter\_no=0$\\
    \While{$iter\_no<T$}{
        $modified\_image=scale(modifier+input\_image)$\\
        $cur=get\_intermediate\_outputs(modified\_image)$\\
        $loss1=dist(modified\_image,input\_image)$\\
        $loss2=get\_loss(des,cur)$\\
        $loss=loss1+c\cdot loss2$\\
        $new\_loss,new\_modifier=Optimizer(loss,modifier)$\\
        $modifier=new\_modifier$\\
        \If{$new\_loss<min\_loss$}{
            $best\_solution=new\_modifier$\\
            $min\_loss=new\_loss$\\
            
        }
        $iter\_no=iter\_no+1$\\
    
    }
    $final\_attacked\_image=best\_solution+input\_image$\\
  
  
  
    
}

\end{algorithm} 

Steps mentioned in figure \ref{fig:approachILFO} (b) can be explained through Algorithm \ref{alg:L2}. The algorithm takes an image to perturb as input ($input\_image$) and returns perturbed image ($final\_attacked\_image$).

\textbf{Initializing Perturbation}: This step is used for initializing variables. We initialize perturbation ($modifier$), minimum loss recorded ($min\_loss$), most successful perturbation ($best\_solution$) and desired state ($des$) (Line 2). Desired state is formulated manually using steps of \ref{fig:approachILFO} (a). Number of iterations ($T$) is also initialized (Line 3). This step is performed only once in the algorithm.

\textbf{Optimizing Loss Function}: This is a step which gets executed for each iteration. A perturbed image ($modified\_image$) is generated by adding perturbation ($modifier$) to the input image ($input\_image$) (Line 6). $scale$ method re-scales the $modified\_image$ using $tanh$ function. Current output state ($cur$) is generated from $get\_intermediate\_outputs$ method using inference of $attacked\_image$ (Line 7). Two types of loss function values are generated. First loss function ($loss1$) measures Euclidean distance between input image ($input\_image$) and perturbed image ($modified\_image$) (Line 8). Second loss function ($loss2$) measures distance between current ($cur$) and desirable ($des$) intermediate output states using $get\_loss$ method (Line 9). $get\_loss$ method is defined during last step of \ref{fig:approachILFO} (a). The main loss function ($loss$) is created using $loss1$ and $loss2$ (Line 10). The main loss function is optimized and updated perturbation ($new\_modifier$) and optimized loss function ($new\_loss$) is generated (Line 11).




\textbf{Update Perturbation and Record Most Successful Perturbation}: Perturbation variable ($modifier$) is updated using $new\_modifier$ (Line 12).
If updated loss ($new\_loss$) is lesser than the recorded minimum loss ($min\_loss$) (Line 13), $min\_loss$ variable is updated (Line 15) and the current solution is recorded as most successful perturbation ($best\_solution$) (Line 14).
$final\_attacked\_image$ is returned as the perturbed output image by adding most successful perturbation ($best\_solution$) with input image ($input\_image$) (Line 19).




\begin{comment}

Algorithm \ref{alg:L2} explains the the ILFO algorithm. The image which we need to perturb is taken as input ($input\_image$). At first, We initialize variables $modifier, min\_loss, best\_solution$ and $des$ in Line 2. Variable $modifier$ represents the distortion that are going to be added to the original image. We initialize it with random values. Variables $min\_loss$ represents minimum loss function value recorded and $best\_solution$ is the modifier responsible for $min\_loss$. Variable $des$ is the desired intermediate output value(s) as discussed earlier in the section \ref{sec:form}.
$T$ is the predefined number of iterations (Line 3).
For each iteration, first we create $attacked\_image$ by adding modifier to the $input\_image$ and $scale$ method re-scales the $attacked\_image$ by using $tanh$ function (Line 6). That $attacked\_image$ is sent for inference and $get\_intermediate\_outputs$ method returns current value(s) of intermediate output(s) as $cur$ (Line 7). Next the algorithm calculates the loss function value. $loss1$ is the euclidean distance between $input\_image$ and $attacked\_image$ which we get from $dist$ method (Line 8). $loss2$ is the difference between $des$ and $cur$ generated by method $get\_loss$ (Line 9). Total loss function value is calculated by the combination of both $loss1$ and $loss2$ where $loss2$ is scaled by constant $c$ (Line 10). Next we call the optimizer which generates an optimized loss function value($new\_loss$) and updates modifier ($new\_mod$) value (Line 11). $modifier$ variable is replaced by $new\_mod$ (Line 12). If the $new\_loss$ is lesser than the minimum loss value recorded ($min\_loss$), we store $new\_loss$ and $new\_mod$ as $min\_loss$ and $best\_solution$ (Line 13-15). After number of iterations exceed $T$, we find the $final\_attacked\_image$ by adding $best\_solution$ to the $input\_image$ (Line 19).  

Steps in the figure \ref{fig:approachILFO} is mentioned in algorithm \ref{alg:L2}. In the algorithm, Line 2 represents \textit{Initializing Perturbation} step, Line 11 represents \textit{Optimize Loss Function} step, Line 12 represents \textit{Updating Perturbation} step and Line 13-15 represents \textit{Recording Most Successful Perturbation} step. $get_loss$ function mentioned in Line 9 is loss function which is defined in pre-defining stage.
%$minimize ||\frac{1}{2} \cdot (tanh(w) + 1)-I||_2^2 $+$c \cdot f(\frac{1}{2} \cdot (tanh(w) + 1)) $
\end{comment}
\subsection{Constraint-based Technique}

Constraint-based technique is designed based on equation \eqref{eq:1}. This technique tries to minimize the distortion while increasing energy consumption is handled by constraints. Constraint-based technique has some shortcomings because it is an optimization technique with non linear constraints. One of the shortcomings is that we can not use large input size. We need to send perturbation values as input of the optimization technique.  We only perturb selected pixels to keep the input size low. Constraint-based technique only perturbs pixels in the border of the image. Changing only border pixels makes sure that the main object of the image does not get perturbed. We divide the technique into four steps.



\textbf{Initializing Output.} This step represents initializing the output of the optimization function \textit{i.e.,} resultant perturbation. The optimization with non-linear constraints may find itself in a local minima without proper Initialization. Initialization is done by randomly generated 100 values for distortion and select the value which generates highest energy increase and has the lowest absolute value. 

\textbf{Creating the constraints.}
In the equation \eqref{eq:1}, the constraint is designed to keep all $\alpha$ values $True$.
 But with our observations from results, we noticed that it is very difficult to make all blocks active simultaneously for every image. Specially for few images, the behaviours of two blocks are totally opposite, \textit{i.e.,} making one block active can make other inactive. So, instead of making all the blocks active, we have tried to make certain number of blocks active. If, $N_G$ represents the number of active blocks in the model then the constraint will be $N_G>=G_{Max}$ where $G_{Max}$ is the predefined desired number of active blocks. 
 
 
 


\textbf{Creating Minimization Function.}
Minimization function has been designed to minimize the difference between original and attacked image. For static perturbation attack, we try to minimize the distortion that is going to be added. For borderline perturbation, we minimize the difference between pixel values of original and distorted image.

\textbf{Calling Optimization Function.}
The optimization function for constraint-based perturbation attack can be represented as,


The optimization function for static perturbation attack can be represented as,


\begin{gather}\label{eq:4}
minimize(||x-x'||)\\
\intertext{such that,} 
\begin{aligned}
(N(x') > G_{Max})
\end{aligned}\notag
%\intertext{and,} 
\end{gather}


Where, $N$ is a method that returns number of active gates, $G_{Max}$ is desired active number of gates, $x'$ is the attacked image with changed borderline pixel values, $x$ is image input.

%$minimize(v)$  $s.t.$  $(WS(I+v) > T)$ and $v < \varepsilon$
\begin{comment}

\begin{gather}\label{eq:3}
minimize(\delta)\\
\intertext{such that,} 
\begin{aligned}
(WS(x+\delta) > T)
\end{aligned}\notag
\intertext{and,} 
\begin{aligned}
\delta < \varepsilon
\end{aligned}\notag
\end{gather}

Where, $\delta$ is distortion added to the full image, $x$ is image input, $WS$ is a method that returns weighted sum $S$ of all gates, $T$ is threshold and $\varepsilon$ is the limit for distortion. Distortion $\delta$ is added to the all image pixels. If after adding $\delta$ the pixel value exceeds maximum or minimum value limit, then that pixel value is clipped to maximum or minimum value.

For borderline perturbation attack, the optimization function is,
\end{comment}
%$minimize(\sum_{k \in K}||I[k]-V[k]||)$  $s.t.$  $(WS(I^\prime) > T)$ 




We have used Sequential Least Squares Programming (SLSQP) to as the optimization algorithm.
 

\begin{comment}
\begin{figure}[t]%
	\centering
	\includegraphics[width=0.53\textwidth]{figures/Approach_cons.pdf}

	\caption{Steps of Constraint-based Technique}
	
	\label{fig:approachcons}
\end{figure}

Instead of formulating the attack as purely optimization technique, constraint-based technique uses optimization function with non-linear constraints for attack. As discussed earlier in this section, distortion and energy consumption are two main factors of formulating the attack. Constraint-based technique uses minimizing distortion as optimization function while constraints are based on intermediate outputs generated from the model. The operations in the AdNN are not linear. Because of this reason, non-linear constraints are used instead of linear constraints. Constraint-based techniques have some limitations. One of them is that constraint-based technique does not perform well when the constraints are dependent on a large number of intermediate outputs. Because of this reason, we implemented constraint based attack only for attacking Conditional-skipping AdNN \footnote{SACT calculates halting score after each layer for each position. Number of intermediate outputs is very high fot SACT}. 
\end{comment}




\begin {comment}
\textbf{Modified L2 Attack.}

L2 is a distance measure which takes euclidean distance between pixel values two images. In this type of attack, small changes are added to many pixels in order to minimize a loss function. The loss function is designed in a way such that minimizing the loss function will eventually lead to higher energy consumption.
Figure \ref{fig:approachcw} represents the work flow of Modified L2 Attack. In this attack also, the initialization of variables are required because the optimizer can find a local minima. Although, it has been noticed from the result that, initial results does not affect the output beyond a certain limit. The loss function has two parts. First part ($l_1$) illustrates the difference in image pixels between original and distorted image. Second part ($l_2$) describes the objective of the operation. In the original L2 attack \ref{fig:approachcw}, $l_2$ was described as the difference between original label and desired label. For Adaptive Neural Networks, $l_2$ will be the difference in current number of computations and desired number of computations. For SkipNet, $l_2$ describes the difference between desired gate outputs and current gate outputs. While, for SACT, $l_2$ is the difference between desired ponder costs of the positions and current ponder costs. After we define the loss function, we use an optimizer to optimize the loss function. 
The optimization function can be written as,

$minimize ||\frac{1}{2} \cdot (tanh(w) + 1)-x||_2^2 $+$c \cdot f(\frac{1}{2} \cdot (tanh(w) + 1)) $

Where, w is the generated perturbation, x is the original image, c is the constant modifying which would decide which part of the loss should be concentrated more and f represents $l_2$. The 




Add example.
\end {comment}

 
\begin{comment}
\begin{figure}[t]%
	\centering
	\includegraphics[width=0.53\textwidth]{figures/resnet_101.pdf}

	\caption{Layers of ResNet-101}
	
	\label{fig:example2}
\end{figure}
\end{comment}
\begin {comment}
1. What is the target of attack? (add a section)
2. minimizing distortion adding in prob formulation.
3. Generic figure. 
4. first line verbose.
5. what does boolean alpha represent.
6. more natural language explanation.
7. Explain ponder cost in problem formulation. (SACT not clear)

\end {comment}

==> proposal.tex <==
\section{Results}
We evaluated our techniques on CIFAR-10 dataset for both SkipNet and SACT models and Imagenet dataset for SkipNet model. The reason for choosing these two datasets is that these models were evaluated used the same datasets to report models' performance. We have processed all the images from CIFAR-10 dataset and chose the images with lower energy consumption and for Imagenet, we chose 100 images with lower energy consumption. The term 'lower energy consumption' is dependent on a threshold which varies for different models. As discussed earlier, SkipNet and SACT both are modified versions of ResNet. SkipNet uses modified ResNet-110 model to classify CIFAR-10 and ResNet-101 model to classify Imagenet images. SACT used ResNet-32 to classify CIFAR-10 images. For ResNet-110, there are 54 residual blocks. We call an image has consumed lower energy if its inference make less than 54 blocks active. Similarly, for ResNet -101, the thesold is 24 out of 33 blocks. For SACT, the lower energy threthan shold is dependent on mean ponder cost. For ResNet-32, if an image's ponder cost is less 11.5, we consider it low energy consuming image. 
\begin{table}[t]
	\scriptsize\center\caption{\label{tab:compare2}  Performmance Eval } 
	\begin{tabular}{|@{\hskip1pt}l@{\hskip1pt}|@{\hskip1pt}r@{\hskip1pt}|@{\hskip1pt}r@{\hskip1pt}|@{\hskip1pt}r@{\hskip1pt}|r@{\hskip1pt}|}
		\hline &  \multicolumn{2}{|c|}{Skipnet}&  \multicolumn{2}{|c|}{SACT}\\\cline{2-5}
		Models&CIFAR-10&Imagenet&CIFAR-10\\\hline\hline
		L2 &30.97\% & 26.97\%&42.4\%\\
		Borderline&7.16\%&11.06\%\%&----\\
		Static &2.85\%&2.99\%&----\\
		\hline
		\end{tabular}
\end{table}

Table \ref{tab:compare2} represents the increase in FLOPs through our attacks in terms of percentage. We can see that L2 attack has outperformed other attacks.
SACT uses ResNet-32 to classify CIFAR-10 and ResNet-101 model to classify Imagenet dataset.

\section{Saving Energy by distortion}

In this section, we would discuss about the possibility of decreasing energy consumption by adding distortion to the image. It would be interesting if we can find an universal distortion which we can add to each image such that the energy consumption of that image will decrease. For this purpose, we need to focus on two points. First, the distortion should not change the output. Second, the distortion should be able decrease energy for all images.  Instead of adding distortion to all pixels, We plan to add a small patch of noise to the image. If we want to change all pixels for the universal distortion, it may not be possible to make image output label intact. So, at first, we will take 500-1000 images from a dataset.
Then, we will find a position of the image whose contribution to the output is less. We can use the technique used in L0 attack proposed by Carlini et. al \cite{carlini2017towards} which finds out pixels which are less relevant for output. After finding the position, we will define a loss function and try to minimize that function. The loss function will have two parts. First part would describe the decrease in energy and second part would be responsible to make outputs intact. Let's assume x is input image and $\delta$ is the patch to be added. We define two intermediate output states $des$ and $cur$. $des$ is the desirable intermediate outputs for which the energy consumption will be 0. $cur$ is current intermediate outputs. First part of the loss function can be defined as,
$f_1(x+\delta)=max(0,des-cur)$

The second part of the loss function is,

$f_2(x+\delta)=loss_{F,t}(x+\delta)$, which describes the entropy loss between current output $t$ and generated output $F$.

The optimization function will be,

\begin{gather}\label{eq:2}
minimize(f_1(x+\delta)+c \cdot f_2(x+\delta))\\
\intertext{such that,} 
\begin{aligned}
(x+\delta) \in [0,1]^n
\end{aligned}\notag
\end{gather}


he $c$ is a suitably chosen constant value and $c>0$.

==> rebuttal.tex <==
\section{Common Issues (Across all reviewers)}

\textbf{Removal of SkipNet from certain experiments.}

\textbf{Usage of FFT.}

\textbf{Threshold in the study.}



\section{Reviewer 1 Issues}


\section{Reviewer 2 Issues}

\section{Reviewer 3 Issues}

==> usecases.tex <==
\section{Use Cases and Threat Model}

For a number of use cases, impact of attacking an AdNN can be unpleasant. People are more inclined to use software applications now and more number of applications are using Machine Learning models for better user experience. All the applications expect fast and accurate result from the models. Attacking AdNN will slowdown the app performance and will affect user experience. For few cases, Attack on AdNN can be as leathal as attackinh traditional DNN. Attacking AdNN while an autonomous car is using AdNN model or visually impaired person is using AdNN model based app while crossing the road can be fatal.
Other than fatality, Attacking AdNN is more `subtle' than attacking traditional DNN because of difficulty in evaluating if an AdNN model is attacked. Changing output through attack is noticeable and can be reported within a short period of time. Increasing response time can be caused by various reasons. So, it would be harder to detect if AdNN model is attacked.

The attack we are proposing is a white-box attack. Attacker will know which AdNN model is being used and will know the architecture and working mechanism of AdNN model in depth. Generating white-box attack against AdNNs is different from generating traditional white-box attacks in this scenario because for attacking DNN, the attacker only needs access to the probabilities in the output layer. For AdNN, attacker needs to find  the target intermediate outputs also is responsible to increase  or decrease FLOPs.
 
